Fluctuation Spectra and Coarse Graining in Stochastic Dynamics

Fluctuations in small biological systems can be crucial for their function. Large-deviation theory characterizes such rare events from the perspective of stochastic processes. In most cases it is very difficult to directly determine the large-deviation functions. Circumventing this necessity, I present a method to quantify the fluctuation spectra for arbitrary Markovian models with finite state space. Under non-equilibrium conditions, current-like observables are of special interest. The space of all current-like observables has a natural decomposition into orthogonal complements. Remarkably, the fluctuation spectrum of any observable is entirely determined by only one of these components. The method is applied to study differences of fluctuations in setups sampling the same dynamics at different resolutions. Coarse graining relates these models and can be done in a way that preserves expectation values of observables. However, the effects of the coarse graining on the fluctuations are not obvious. These differences are explicitly worked out for a simple model system.

==> abstract_nomenclature.tex <==
\begin{abstract}
  Things to be said in an abstract.
  \bigskip\par
  \textbf{Keywords:} statistical physics, Markovian jump processes, non-equilibrium phenomena, non-equilibrium fluctuations in small systems, large deviations in non-equilibrium systems,

\end{abstract}
%%% So laesst sich in die andere Sprache umschalten (Englisch bzw. Deutsch)
%\begin{otherlanguage}{ngerman}
%\begin{abstract}
%Hier werden auf einer halben Seite die Kernaussagen der Arbeit
%  zusammengefasst.
%%% Optional: Stichwoerter. Wenn nicht gewuenscht, koennen die beiden
%%% folgenden Zeilen geloescht werden
%  \bigskip\par
%  \textbf{Stichwörter:} Physik, Bachelorarbeit
%\end{abstract}
%\end{otherlanguage}

%% Hier kann man seine Bezeichnungsweisen erklaeren. Falls nicht
%% benoetigt, bis einschliesslich \end{nomenclature} auskommentieren
%\begin{nomenclature}
%%% Fuer die Berechnung der Spaltenbreiten muss \usepackage{calc}
%%% geladen sein!
%\section*{Lateinische Buchstaben}
%\noindent
%\begin{longtable}[l]{p{0.2\textwidth}p{0.7\textwidth-6\tabcolsep}p{0.1\textwidth}}
%  \tabheadfont{Variable}&\tabheadfont{Bedeutung}&\tabheadfont{Einheit}\\\midrule\endhead
%  $A$ & Querschnittsfläche & $\unit{}{\squaren\meter}$\\
%  $c$ & Geschwindigkeit & $\unit{}{\meter\per\second}$
%\end{longtable}
%\section*{Griechische Buchstaben}
%\begin{longtable}[l]{p{0.2\textwidth}p{0.7\textwidth-6\tabcolsep}p{0.1\textwidth}}
%  \tabheadfont{Variable}&\tabheadfont{Bedeutung}&\tabheadfont{Einheit}\\\midrule\endhead
%  $\alpha$  & Winkel & $\unit{}{\degree}$; --\\
%  $\varrho$ & Dichte & $\unit{}{\kilo\gram\per\cubic\meter}$
%\end{longtable}
%\section*{Indizes}
%\begin{longtable}[l]{p{0.2\textwidth}p{0.8\textwidth-4\tabcolsep}}
%  \tabheadfont{Index}&\tabheadfont{Bedeutung}\\\midrule\endhead
%  m & Meridian\\
%  $r$ & Radial
%\end{longtable}
%\section*{Abkürzungen}
%\begin{longtable}[l]{p{0.2\textwidth}p{0.8\textwidth-4\tabcolsep}}
%  \tabheadfont{Abkürzung}&\tabheadfont{Bedeutung}\\\midrule\endhead
%  2D & zweidimensional\\
%  3D & dreidimensional\\
%  max & maximal
%\end{longtable}
%\end{nomenclature}
%% \listoftables und \listoffigures sollten nur bei genuegender Anzahl Tabellen
%% verwendet werden
%\listoffigures
%\listoftables


==> hyphenation.tex <==
\hyphenation{Gärt-ner--Ellis}
\hyphenation{Wojt-kow-ski}


==> packages.tex <==
\usepackage[utf8]{inputenc}

\usepackage{float}

% language option set in JGNSUM class
\usepackage[english]{babel}

%% FONT:
\usepackage{lmodern}


%\usepackage{times} % sieht besser aus als lmodern
%\usepackage{palatino} % sieht schlechter aus als times
%\usepackage{mathpazo} % very ugly font, to be loaded later ???
%\usepackage{cmbright} % doesn't work either
%\usepackage[utopia]{mathdesign}
%\usepackage[urw-garamond]{mathdesign}
\usepackage{libertine}
\usepackage{fourier}
%\usepackage{dsfont}
\usepackage[T1]{fontenc}
%\usepackage{mathdots}
\usepackage{amsfonts}
\usepackage{amstext}
\usepackage{amsmath}
%\usepackage{amsthm}
\usepackage{amssymb}
%\usepackage{amsbsy}   % AMS-Boldsymbol
\usepackage[amsmath,thref]{ntheorem}
\usepackage{bbm}
%\usepackage{array}
\usepackage{siunitx}

%\usepackage{wrapfig}
\usepackage{graphicx}

%\usepackage{textcomp} % noch einige coole symbole

%\usepackage{sectsty}
%\allsectionsfont{\raggedright}

%\usepackage{makeidx}

\usepackage{url}	% für hübsche URLs mit Link
\usepackage{color}	% für farben a la \definecolor{Gray}{gray}{0.5}

%\usepackage{fancybox}
\usepackage{icomma}
%\usepackage{nicefrac}
%\usepackage{forloop}
\usepackage{xspace}
\usepackage{uniinput}

%\usepackage[comma,numbers,sort&compress]{natbib}
%\bibliographystyle{plainat}

\usepackage[sectionbib,square]{natbib}
\bibliographystyle{arturstyle}
\citestyle{plain}
%\bibliographystyle{plainnat}
%\bibliographystyle{plainnat}
%\bibliographystyle{abbrvnat}
%\bibliographystyle{apalike}
%\bibliographystyle{unsrtnat}

\usepackage[colorlinks,pdftex]{hyperref}

